Reduced order models from computed states of physical systems using non-local calculus on finite weighted graphs

Partial differential equation-based numerical solution frameworks for initial and boundary value problems have attained a high degree of complexity. Applied to a wide range of physics with the ultimate goal of enabling engineering solutions, these approaches encompass a spectrum of spatiotemporal discretization techniques that leverage solver technology and high performance computing. While high-fidelity solutions can be achieved using these approaches, they come at a high computational expense and complexity. Systems with billions of solution unknowns are now routine. The expense and complexity do not lend themselves to typical engineering design and decision-making, which must instead rely on reduced-order models. Here we present an approach to reduced-order modelling that builds off of recent graph theoretic work for representation, exploration, and analysis on computed states of physical systems (Banerjee et al., Comp. Meth. App. Mech. Eng., 351, 501-530, 2019). We extend a non-local calculus on finite weighted graphs to build such models by exploiting first order dynamics, polynomial expansions, and Taylor series. Some aspects of the non-local calculus related to consistency of the models are explored. Details on the numerical implementations and the software library that has been developed for non-local calculus on graphs are described. Finally, we present examples of applications to various quantities of interest in mechano-chemical systems.

==> figures/model_psi_OLS.tex <==
${\Psi}_{} = {{\Psi}_{}}_{0} + {\gamma}^{{\bar{\varphi}}_{}{\bar{\varphi}}_{}}\frac{1}{2!}\frac{{\delta}^{2} {\Psi}_{}({{\mathbf{\bar{E}}}}_{0},{{{\bar{\varphi}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2}}{\Delta {\bar{\varphi}}_{}}^{2} + {\gamma}^{{\bar{E}}_{12}{\bar{\varphi}}_{}}\frac{1}{2!}\frac{{\delta}^{2} {\Psi}_{}({{\mathbf{\bar{E}}}}_{0},{{{\bar{\varphi}}}}_{0})}{\delta {\bar{E}}_{12} \delta {\bar{\varphi}}_{}}{\Delta {\bar{E}}_{12}}^{} {\Delta {\bar{\varphi}}_{}}^{} + {\gamma}^{{\bar{E}}_{12}{\bar{\varphi}}_{}{\bar{\varphi}}_{}}\frac{1}{3!}\frac{{\delta}^{3} {\Psi}_{}({{\mathbf{\bar{E}}}}_{0},{{{\bar{\varphi}}}}_{0})}{\delta {\bar{E}}_{12} \delta {\bar{\varphi}}_{} \delta {\bar{\varphi}}_{}}{\Delta {\bar{E}}_{12}}^{} {\Delta {\bar{\varphi}}_{}}^{2} + {\gamma}^{{\bar{E}}_{11}{\bar{E}}_{22}}\frac{1}{2!}\frac{{\delta}^{2} {\Psi}_{}({{\mathbf{\bar{E}}}}_{0},{{{\bar{\varphi}}}}_{0})}{\delta {\bar{E}}_{11} \delta {\bar{E}}_{22}}{\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{} + {\gamma}^{{\bar{\varphi}}_{}{\bar{E}}_{22}{\bar{E}}_{11}}\frac{1}{3!}\frac{{\delta}^{3} {\Psi}_{}({{\mathbf{\bar{E}}}}_{0},{{{\bar{\varphi}}}}_{0})}{\delta {\bar{\varphi}}_{} \delta {\bar{E}}_{22} \delta {\bar{E}}_{11}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{22}}^{} {\Delta {\bar{E}}_{11}}^{} + {\gamma}^{{\bar{E}}_{11}{\bar{E}}_{22}{\bar{\varphi}}_{}{\bar{\varphi}}_{}}\frac{1}{4!}\frac{{\delta}^{4} {\Psi}_{}({{\mathbf{\bar{E}}}}_{0},{{{\bar{\varphi}}}}_{0})}{\delta {\bar{E}}_{11} \delta {\bar{E}}_{22} \delta {\bar{\varphi}}_{} \delta {\bar{\varphi}}_{}}{\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{} {\Delta {\bar{\varphi}}_{}}^{2} + {\gamma}^{{\bar{E}}_{22}{\bar{\varphi}}_{}}\frac{1}{2!}\frac{{\delta}^{2} {\Psi}_{}({{\mathbf{\bar{E}}}}_{0},{{{\bar{\varphi}}}}_{0})}{\delta {\bar{E}}_{22} \delta {\bar{\varphi}}_{}}{\Delta {\bar{E}}_{22}}^{} {\Delta {\bar{\varphi}}_{}}^{} + {\gamma}^{{\bar{E}}_{11}{\bar{\varphi}}_{}}\frac{1}{2!}\frac{{\delta}^{2} {\Psi}_{}({{\mathbf{\bar{E}}}}_{0},{{{\bar{\varphi}}}}_{0})}{\delta {\bar{E}}_{11} \delta {\bar{\varphi}}_{}}{\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{\varphi}}_{}}^{} + {\gamma}^{{\bar{\varphi}}_{}{\bar{\varphi}}_{}{\bar{E}}_{22}}\frac{1}{3!}\frac{{\delta}^{3} {\Psi}_{}({{\mathbf{\bar{E}}}}_{0},{{{\bar{\varphi}}}}_{0})}{\delta {\bar{\varphi}}_{} \delta {\bar{\varphi}}_{} \delta {\bar{E}}_{22}}{\Delta {\bar{\varphi}}_{}}^{2} {\Delta {\bar{E}}_{22}}^{}$

==> figures/model_psi_Ridge17.tex <==
${\Psi}_{} = {{\Psi}_{}}_{0} + {\gamma}^{{\bar{\varphi}}_{}{\bar{\varphi}}_{}}\frac{1}{2!}\frac{{\delta}^{2} {\Psi}_{}({{\mathbf{\bar{E}}}}_{0},{{{\bar{\varphi}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{2}}{\Delta {\bar{\varphi}}_{}}^{2} + {\gamma}^{{\bar{\varphi}}_{}{\bar{\varphi}}_{}{\bar{\varphi}}_{}{\bar{\varphi}}_{}}\frac{1}{4!}\frac{{\delta}^{4} {\Psi}_{}({{\mathbf{\bar{E}}}}_{0},{{{\bar{\varphi}}}}_{0})}{{\delta {\bar{\varphi}}_{}}^{4}}{\Delta {\bar{\varphi}}_{}}^{4} + {\gamma}^{{\bar{\varphi}}_{}{\bar{E}}_{22}{\bar{E}}_{11}}\frac{1}{3!}\frac{{\delta}^{3} {\Psi}_{}({{\mathbf{\bar{E}}}}_{0},{{{\bar{\varphi}}}}_{0})}{\delta {\bar{\varphi}}_{} \delta {\bar{E}}_{22} \delta {\bar{E}}_{11}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{22}}^{} {\Delta {\bar{E}}_{11}}^{} + {\gamma}^{{\bar{\varphi}}_{}{\bar{E}}_{11}{\bar{E}}_{11}{\bar{E}}_{11}}\frac{1}{4!}\frac{{\delta}^{4} {\Psi}_{}({{\mathbf{\bar{E}}}}_{0},{{{\bar{\varphi}}}}_{0})}{\delta {\bar{\varphi}}_{} \delta {\bar{E}}_{11} \delta {\bar{E}}_{11} \delta {\bar{E}}_{11}}{\Delta {\bar{\varphi}}_{}}^{} {\Delta {\bar{E}}_{11}}^{3} + {\gamma}^{{\bar{E}}_{11}{\bar{E}}_{22}}\frac{1}{2!}\frac{{\delta}^{2} {\Psi}_{}({{\mathbf{\bar{E}}}}_{0},{{{\bar{\varphi}}}}_{0})}{\delta {\bar{E}}_{11} \delta {\bar{E}}_{22}}{\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{E}}_{22}}^{} + {\gamma}^{{\bar{E}}_{12}}\frac{{\delta}^{} {\Psi}_{}({{\mathbf{\bar{E}}}}_{0},{{{\bar{\varphi}}}}_{0})}{{\delta {\bar{E}}_{12}}^{}}{\Delta {\bar{E}}_{12}}^{} + {\gamma}^{{\bar{E}}_{11}{\bar{\varphi}}_{}}\frac{1}{2!}\frac{{\delta}^{2} {\Psi}_{}({{\mathbf{\bar{E}}}}_{0},{{{\bar{\varphi}}}}_{0})}{\delta {\bar{E}}_{11} \delta {\bar{\varphi}}_{}}{\Delta {\bar{E}}_{11}}^{} {\Delta {\bar{\varphi}}_{}}^{} + {\gamma}^{{\bar{E}}_{22}{\bar{\varphi}}_{}}\frac{1}{2!}\frac{{\delta}^{2} {\Psi}_{}({{\mathbf{\bar{E}}}}_{0},{{{\bar{\varphi}}}}_{0})}{\delta {\bar{E}}_{22} \delta {\bar{\varphi}}_{}}{\Delta {\bar{E}}_{22}}^{} {\Delta {\bar{\varphi}}_{}}^{} + {\gamma}^{{\bar{\varphi}}_{}{\bar{\varphi}}_{}{\bar{E}}_{22}}\frac{1}{3!}\frac{{\delta}^{3} {\Psi}_{}({{\mathbf{\bar{E}}}}_{0},{{{\bar{\varphi}}}}_{0})}{\delta {\bar{\varphi}}_{} \delta {\bar{\varphi}}_{} \delta {\bar{E}}_{22}}{\Delta {\bar{\varphi}}_{}}^{2} {\Delta {\bar{E}}_{22}}^{}$

==> figures/model_vol_OLS_0_1.tex <==
\begin{align}
\frac{{\delta}^{} {\bar{\varphi}}_{\textrm{OLS}}}{{\delta} {{{t}}_{}}^{}} =&~ {\gamma}^{({{\bar{E}}_{11}})^{}({{\bar{E}}_{12}})^{}({{\bar{l}}_{1}})^{}}({{\bar{E}}_{11}})^{} ({{\bar{E}}_{12}})^{} ({{\bar{l}}_{1}})^{} + {\gamma}^{({{\bar{E}}_{12}})^{}({{\bar{\varphi}}_{}})^{}({{\bar{l}}_{1}})^{}}({{\bar{E}}_{12}})^{} ({{\bar{\varphi}}_{}})^{} ({{\bar{l}}_{1}})^{} \label{eq:vol_square_1_model_OLSlstsq} \\
+&~ {\gamma}^{({{\bar{E}}_{11}})^{}({{\bar{E}}_{22}})^{}({{\bar{l}}_{2}})^{}}({{\bar{E}}_{11}})^{} ({{\bar{E}}_{22}})^{} ({{\bar{l}}_{2}})^{} + {\gamma}^{({{\bar{E}}_{11}})^{}({{\bar{E}}_{22}})^{}}({{\bar{E}}_{11}})^{} ({{\bar{E}}_{22}})^{} \nonumber \\ 
+&~  {\gamma}^{({{\bar{E}}_{22}})^{2}}({{\bar{E}}_{22}})^{2} + {\gamma}^{({{\bar{E}}_{22}})^{2}({{\bar{l}}_{2}})^{}}({{\bar{E}}_{22}})^{2} ({{\bar{l}}_{2}})^{} \nonumber \\ 
+&~  {\gamma}^{({{\bar{\varphi}}_{}})^{}({{\bar{l}}_{1}})^{}}({{\bar{\varphi}}_{}})^{} ({{\bar{l}}_{1}})^{} + {\gamma}^{({{\bar{\varphi}}_{}})^{2}({{\bar{l}}_{1}})^{}}({{\bar{\varphi}}_{}})^{2} ({{\bar{l}}_{1}})^{} \nonumber \\ 
+&~  {\gamma}^{({{\bar{E}}_{11}})^{2}({{\bar{l}}_{1}})^{}}({{\bar{E}}_{11}})^{2} ({{\bar{l}}_{1}})^{} + {\gamma}^{({{\bar{E}}_{11}})^{}({{\bar{l}}_{1}})^{}}({{\bar{E}}_{11}})^{} ({{\bar{l}}_{1}})^{} \nonumber
\end{align}

==> figures/model_vol_OLSorig_0_1.tex <==
\begin{align}
\frac{{\delta}^{} {\bar{\varphi}}_{}}{{\delta} {{{t}}_{}}^{}} ~=~&~ {\gamma}^{({{\bar{E}}_{11}})^{}({{\bar{\varphi}}_{}})^{}({{\bar{N}}_{1}})^{}}({{\bar{E}}_{11}})^{} ({{\bar{\varphi}}_{}})^{} ({{\bar{N}}_{1}})^{} + {\gamma}^{({{\bar{E}}_{11}})^{2}({{\bar{N}}_{1}})^{}}({{\bar{E}}_{11}})^{2} ({{\bar{N}}_{1}})^{} \label{eq:vol_square_1_model_OLSorig} \\
+&~{\gamma}^{({{\bar{E}}_{22}})^{}({{\bar{\varphi}}_{}})^{}({{\bar{N}}_{1}})^{}}({{\bar{E}}_{22}})^{} ({{\bar{\varphi}}_{}})^{} ({{\bar{N}}_{1}})^{} + {\gamma}^{({{\bar{E}}_{11}})^{}({{\bar{E}}_{22}})^{}({{\bar{N}}_{1}})^{}}({{\bar{E}}_{11}})^{} ({{\bar{E}}_{22}})^{} ({{\bar{N}}_{1}})^{} \nonumber \\ 
+&~ {\gamma}^{({{\bar{E}}_{22}})^{}({{\bar{\varphi}}_{}})^{}({{\bar{l}}_{1}})^{}}({{\bar{E}}_{22}})^{} ({{\bar{\varphi}}_{}})^{} ({{\bar{l}}_{1}})^{} + {\gamma}^{({{\bar{E}}_{11}})^{}({{\bar{E}}_{22}})^{}({{\bar{l}}_{1}})^{}}({{\bar{E}}_{11}})^{} ({{\bar{E}}_{22}})^{} ({{\bar{l}}_{1}})^{}  \nonumber \\
+&~ {\gamma}^{({{\bar{E}}_{11}})^{}({{\bar{\varphi}}_{}})^{}({{\bar{l}}_{1}})^{}}({{\bar{E}}_{11}})^{} ({{\bar{\varphi}}_{}})^{} ({{\bar{l}}_{1}})^{} + {\gamma}^{({{\bar{E}}_{11}})^{2}({{\bar{l}}_{1}})^{}}({{\bar{E}}_{11}})^{2} ({{\bar{l}}_{1}})^{}  \nonumber \\
+&~ {\gamma}^{({{\bar{E}}_{11}})^{}({{\bar{\varphi}}_{}})^{}({{\bar{l}}_{2}})^{}}({{\bar{E}}_{11}})^{} ({{\bar{\varphi}}_{}})^{} ({{\bar{l}}_{2}})^{} + {\gamma}^{({{\bar{E}}_{11}})^{}({{\bar{\varphi}}_{}})^{}}({{\bar{E}}_{11}})^{} ({{\bar{\varphi}}_{}})^{}. \nonumber
\end{align}

==> figures/model_vol_Ridge17_0_1.tex <==
\begin{align}
\frac{{\delta}^{} {\bar{\varphi}}_{\textrm{Ridge}}}{{\delta} {{{t}}_{}}^{}} =&~ {\gamma}^{({{\bar{E}}_{11}})^{}({{\bar{E}}_{12}})^{}}({{\bar{E}}_{11}})^{} ({{\bar{E}}_{12}})^{} + {\gamma}^{({{\bar{E}}_{12}})^{}({{\bar{l}}_{1}})^{}}({{\bar{E}}_{12}})^{} ({{\bar{l}}_{1}})^{} \label{eq:vol_square_1_model_Ridge17} \\
+&~ {\gamma}^{({{\bar{E}}_{11}})^{2}}({{\bar{E}}_{11}})^{2} + {\gamma}^{({{\bar{E}}_{11}})^{2}({{\bar{l}}_{2}})^{}}({{\bar{E}}_{11}})^{2} ({{\bar{l}}_{2}})^{} \nonumber \\ 
+&~  {\gamma}^{({{\bar{E}}_{22}})^{}({{\bar{l}}_{2}})^{}}({{\bar{E}}_{22}})^{} ({{\bar{l}}_{2}})^{} + {\gamma}^{({{\bar{E}}_{22}})^{2}}({{\bar{E}}_{22}})^{2} \nonumber \\ 
+&~  {\gamma}^{({{\bar{E}}_{11}})^{}}({{\bar{E}}_{11}})^{} + {\gamma}^{({{\bar{E}}_{12}})^{}({{\bar{E}}_{22}})^{}({{\bar{l}}_{1}})^{}}({{\bar{E}}_{12}})^{} ({{\bar{E}}_{22}})^{} ({{\bar{l}}_{1}})^{} \nonumber \\ 
+&~ {\gamma}^{({{\bar{\varphi}}_{}})^{2}({{\bar{l}}_{1}})^{}}({{\bar{\varphi}}_{}})^{2} ({{\bar{l}}_{1}})^{} +  {\gamma}^{({{\bar{E}}_{11}})^{}({{\bar{E}}_{22}})^{}({{\bar{l}}_{1}})^{}}({{\bar{E}}_{11}})^{} ({{\bar{E}}_{22}})^{} ({{\bar{l}}_{1}})^{} \nonumber
\end{align}

